I2I: Initializing Adapters with Improvised Knowledge

Adapters present a promising solution to the catastrophic forgetting problem in continual learning. However, training independent Adapter modules for every new task misses an opportunity for cross-task knowledge transfer. We propose Improvise to Initialize (I2I), a continual learning algorithm that initializes Adapters for incoming tasks by distilling knowledge from previously-learned tasks' Adapters. We evaluate I2I on CLiMB, a multimodal continual learning benchmark, by conducting experiments on sequences of visual question answering tasks. Adapters trained with I2I consistently achieve better task accuracy than independently-trained Adapters, demonstrating that our algorithm facilitates knowledge transfer between task Adapters. I2I also results in better cross-task knowledge transfer than the state-of-the-art AdapterFusion without incurring the associated parametric cost.

==> tables/forward_transfer.tex <==
\begin{table*}[]
\centering
\small
\begin{tabular}{lcccccccc}
\toprule
\multicolumn{9}{c}{Forward Transfer Results} \\
\midrule
& \multicolumn{6}{c}{Individual Task Transfer, $\knowledgetransfer{i}$} & & \\
\cmidrule{2-7}
Method & \multicolumn{1}{c}{VQA} & \multicolumn{1}{c}{OK-VQA} & \multicolumn{1}{c}{VQA-Abs} & \multicolumn{1}{c}{PathVQA} & \multicolumn{1}{c}{COCO-QA} & \multicolumn{1}{c}{VizWiz} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Average Knowledge \\ Transfer, $\mathbb{T}_{\textit{K}}$\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Average \\ Acc. $\tilde{S}_{\fusion}$\end{tabular}} \\
\midrule
Vanilla Adapters & 1.55 & -4.82   & -1.01   & -0.93 & 4.85  & 1.57 & -0.07  $\pm$ 3.57  & 58.72   \\
%\multicolumn{9}{c}{Average Forward Transfer, across Three Task Orders}\\
\midrule
AdapterFusion  & 1.56  & 8.37 & -1.97   & -1.77 & 3.20  & 2.34 & 1.96 $\pm$ 1.05  & 58.92  $\pm$ 0.45\\
IAO LLF  & 1.73 & 25.60   & -2.86   & -4.40 & 4.55  & 1.50 & \textbf{4.35 $\pm$ 6.12}  & 59.36 $\pm$ 1.60 \\
IAO FLF  & 2.20 & 36.14   & -0.57   & -2.02 & 2.98  & 3.42 & \textbf{7.03 $\pm$ 3.52}  & \textbf{60.33 $\pm$ 0.88}  \\
IAO FFF  & 2.18 & 35.85   & -0.38   & -1.14 & 3.13  & 3.25 & \textbf{7.15 $\pm$ 3.54}  & \textbf{60.44 $\pm$ 0.91}  \\
\bottomrule
\end{tabular}
\label{}
\caption{For every task $i$ we report the knowledge transfer $\knowledgetransfer{i}$, averaged across three different task orders. We also report the overall knowledge transfer $\mathbb{T}_{\textit{K}}$ and average accuracy $S_\fusion$ (mean and standard deviation reported across three three task orders). }
\end{table*}

==> tables/params.tex <==
\begin{comment}
\begin{table*}[t]
    \centering
    %\small
    \begin{tabular}{lrrr}
    %\multicolumn{7}{c}{Fusion Transfer Results} \\
     & \bf \# Task-Specific Params & \bf \# Adapter Params & \\
    \bf Model Configuration & \bf  $\bigl( \sum_k |\Phi_k| + |\Psi_k| \bigr)$ & $\bigl( \sum_k |\Phi_k| \bigr)$ & \bf \# Model Params\\
    \midrule
    CLIP-BART & -- & -- & 227M \\
    \quad + Vanilla Adapters & 10.4M & 4.5M & 237.3M \\ 
    \quad + AdapterFusion & 95.4M & 89.5M & 322.27M \\
    \quad + \algoshort\ & 10.4M & 4.5M & 237.3M \\
    \bottomrule
    \end{tabular}
    \caption{We report the impact of adding task-specific parameters $\Phi_k$ and $\Phi_k$ to CLIP-BART for our 5 VQA tasks with vanilla Adapters, AdapterFusion, and our proposed \algoshort\ algorithm.}
    \label{tab:num_params}
\end{table*}
\end{comment}
\begin{table*}[t]
    \centering
    %\small
    \begin{tabular}{lrrrrr}
    %\multicolumn{7}{c}{Fusion Transfer Results} \\
     & \multicolumn{5}{c}{\bf Model Parameters} \\
     \cmidrule{2-6}
    \bf Model Configuration & \bf Total  & \bf Adapters $|\Phi_k|$ & \bf Fusion $|\fusion_k|$ & \bf All Task-Specific & \bf Single-Task  \\
    & & $\bigl( \sum_k |\Phi_k| \bigr)$ & $\bigl( \sum_k |\fusion_k| \bigr)$ & $\bigl( \sum_k |\Phi_k| + |\fusion_k| + |\Psi_k| \bigr)$ & \bf Inference \\
     %& \bf \# Task-Specific Params & \bf \# Adapter Params & & \# Trainable & \# Inference \\
    %\bf Model Configuration & \bf  $\bigl( \sum_k |\Phi_k| + |\Psi_k| \bigr)$ & $\bigl( \sum_k |\Phi_k| + |\fusion_k| \bigr)$ & \bf \# Model Params & Params & Params \\
    \midrule
    CLIP-BART & 227M & -- & -- & -- & 227M \\
    \quad + Vanilla Adapters & 237.3M & 4.5M & -- & 10.4M & 229.1M \\ 
    \quad + AdapterFusion & 322.3M & 4.5M & 85M & 95.4M & 258.4M \\
    \quad + \algoshort\ & 237.3M & 4.5M & -- & 10.4M & 229.1M \\
    \bottomrule
    \end{tabular}
    \caption{We report the impact of adding task-specific parameters $\Phi_k$ and $\Phi_k$ to CLIP-BART for our 5 VQA tasks with vanilla Adapters, AdapterFusion, and our proposed \algoshort\ algorithm.}
    \label{tab:num_params}
\end{table*}
